iHuman: Instant Animatable Digital Humans From Monocular Videos

Personalized 3D avatars require an animatable representation of digital humans. Doing so instantly from monocular videos offers scalability to broad class of users and wide-scale applications. In this paper, we present a fast, simple, yet effective method for creating animatable 3D digital humans from monocular videos. Our method utilizes the efficiency of Gaussian splatting to model both 3D geometry and appearance. However, we observed that naively optimizing Gaussian splats results in inaccurate geometry, thereby leading to poor animations. This work achieves and illustrates the need of accurate 3D mesh-type modelling of the human body for animatable digitization through Gaussian splats. This is achieved by developing a novel pipeline that benefits from three key aspects: (a) implicit modelling of surface's displacements and the color's spherical harmonics; (b) binding of 3D Gaussians to the respective triangular faces of the body template; (c) a novel technique to render normals followed by their auxiliary supervision. Our exhaustive experiments on three different benchmark datasets demonstrates the state-of-the-art results of our method, in limited time settings. In fact, our method is faster by an order of magnitude (in terms of training time) than its closest competitor. At the same time, we achieve superior rendering and 3D reconstruction performance under the change of poses.

==> pseudo-code.tex <==

\begin{framed}

\begin{lstlisting}[language=Python, caption=Compact Pseudocode for Mesh Processing]

subdiv_mesh()  # Subdivide mesh and blend weights
assign_blend_weights()
for face in mesh: # Init Gaussian splatting vars
    sx, sy, sz, rot, opac, sh_coeffs  = inIt(face)
    
for img, pose in frames:
    v_disps = init_v_disps(norm_verts)     # Init vertex displacements
    deform_mesh = apply_v_disp(mesh, v_disps)    # Displace the mesh
    posed_mesh = apply_lbs(deform_mesh, pose)    # Apply LBS 
    normals, centroids = compute_NC(posed_mesh)  # Normals & centroids
    sh_norms = encode_normals(normals)  # Encode normals with SH
    
    # Gaussian splatting for image and normals
    pred_img = gauss_splat(centroids, shs, scales, rot, opac)
    pred_norm = gauss_splat(centroids, sh_norms, rot, scales)
    
    # Calculate error and optimize
    loss = calc_loss(tgt_img, pred_img) + calc_loss(tgt_norm, pred_norm)
    optimize(loss)
\end{lstlisting}
\end{framed}

==> sections/experiments_old.tex <==

\section{Experiments}
\label{sec:experiments_old}

% NOVEL VIEW SYSNTHESIS: 
% Anim-Nerf Instant Avatar, Neural Body(Maybe)
% PNSR, LPIPS, SSIM
% Poeple, NeuMan
% time: 1hr cutoff
% no of views: 20+ frames (skip : 20, 24)

% NOVEL POSE SYNTHESIS:
% Anim-Nerf Instant Avatar, Neural Body(Maybe)
% PSNR, LPIPS, SSIM
% People, NeuMan


% 3D GEOMETRY LOSS
% Self-Recon, vid2Avatar
% chamfer loss, eclidean distance
% MGN, 3DPW

\subsection{Implementation Details}

\subsection{Dataset}

We evaluate our method on 4 different datasets. \\
similar to that of AnimNerf [@cite] \\

a. The datasets People-Snapshot[@cite] comprise various monocular RGB videos recorded in natural settings. In these videos, individuals assume an A-pose and rotate in place facing a stationary camera.\\

b. The Multi-Garment dataset features 3D scanned models of the human body complete with textures, along with corresponding SMPLD models that are registered for use in animation. For the creation of the videos, we chose x human body models. These models were animated based on motion sequences from the People-Snapshot dataset, where subjects rotate in an A-pose. \\

c. For evaluating our approach in more demanding situations, we utilize outdoor series from the NeuMan dataset [@cite], which consists of videos captured with a mobile phone camera featuring individuals in motion. Specifically, we handpicked four sequences (bike, citron, seattle, jogging) that display the greatest number of body regions and include the fewest number of blurred images. \\

d. 3DPW: for 3d reconstruction. pose and rotate the model like in people snaphsot and generate data \\

d. People Snapshot, NeuMan are used mainly for novel view and novel pose synthesis. And the synthetic data from Multi-Garment dataset are used to evaluate the quality of the 3D reconstructions.

\subsection{Evaluation}

For novel view synthesis, we animate and render the reconstructed model with the poses of test frames in PeopleSnapshot, iPer, and measure the difference between the generated images and the real images.

\textbf{Novel view and pose synthesis} \\
peak signal-to-noise ratio (PSNR), structural similarity index (SSIM [@cite]), and learned perceptual image patch similarity (LPIPS \cite{zhang2018unreasonable}) 
\\

\textbf{3D Reconstruction}\\
point-to-surface Euclidean distance (P2S) and Chamfer distance [@cite] between the reconstructed and the ground truth surfaces
\\

\textbf{Mesh Recovery}
Compare with SuGaR, by providing the canonical space Gaussians without normal loss. Show qualitative difference in quality around hand regions and legs. 

Also, note down the time difference. 

\textbf{Baselines} \\
a. AnimNerf \\
b. InstantAvatar \\
c. Video Based Reconstruction of 3D People/Octopus \\
d. SelfRecon \\
e. Vid2Avatar \\

\subsection{Comparison with SoTA}

\subsubsection{View Reconstruction Quality} \\
a. After full convergence, we show the view reconstruction quality and speed differences compared to SoTA in table \ref{tab:novel_view_synthesis} and figure \ref{fig:novel_view}. \\
b. Comparison with other methods \ref{fig:novel_view_comparison}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/novel_view_placeholder.png}
    \caption{Results of Novel View Synthesis on iPER, PeopleSnapshot & Neuman}
    \label{fig:novel_view}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/novel_view_comparison_placeholder.png}
    \caption{Qualitative Results on }
    \label{fig:novel_view_comparison}
\end{figure}

\begin{table}[h]
\centering
\caption{Placeholder: Qualitative Comparison with SoTA on the PeopleSnapshot [@cite] dataset and iPER dataset for 3-3 subjects. We report PSNR, SSIM, and LPIPS [@cite] between real images and the images generated by InstantAvatar and two SoTA methods and Anim-NeRF [@cite].}
\begin{tabular}{lllllllllllll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Methods}} & \multicolumn{3}{l}{male-3} & \multicolumn{3}{l}{female-3} & \multicolumn{3}{l}{sub-3} & \multicolumn{3}{l}{sub-7} \\
\multicolumn{1}{c}{}                         & PSNR    & SSIM   & LPIPS   & PSNR    & SSIM    & LPIPS    & PSNR    & SSIM    & LPIPS    & PSNR    & SSIM    & LPIPS    \\
\hline
Neural Body(13 hours)                   &         &        &         &         &         &          &         &         &          &         &         &          \\
Anim-Nerf(12 hours)                   &         &        &         &         &         &          &         &         &          &         &         &          \\
Instant Avatar(5 minutes)                    &         &        &         &         &         &          &         &         &          &         &         &          \\
GART(26 views, 20s)                &         &        &         &         &         &          &         &         &          &         &         &          \\
Ours(80s)                                        &         &        &         &         &         &          &         &         &          &         &         &          \\
\hline
Neural Body(26 views, 10mins)                   &         &        &         &         &         &          &         &         &          &         &         &          \\

Anim-Nerf(26 views, 10mins)                  &         &        &         &         &         &          &         &         &          &         &         &          \\
Instant Avatar(26 views, 20s)                &         &        &         &         &         &          &         &         &          &         &         &          \\
GART(26 views, 20s)                &         &        &         &         &         &          &         &         &          &         &         &          \\
Ours(26 views, 20s)                       &         &        &         &         &         &          &         &         &          &         &         &          \\   

\hline
\end{tabular}
\end{table}


\subsubsection{3D Geometry Reconstruction} \\
a. Show geometry reconstruction  similar to \ref{fig:geometry_recon}.\\
b. Create comparison similar to \ref{fig:geometry_recon_comparison}.\\
c. Create table with p2s and chamfer distance on dataset multi garment. \ref{tab:3d_reconstruction_comparison} \\
d. vertex 2 vertex error visualization as in \ref{fig:geometry_error} \\

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/geometry_recon_placeholder.png}
    \caption{Our reconstruction result on ... datasets}
    \label{fig:geometry_recon}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/geometry_recon_comparison_placeholder.png}
    \caption{Qualitative comparison with Anim-Nerf, Video Based 3D People Methods}
    \label{fig:geometry_recon_comparison}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{figures/geometry_error_placeholder.png}
    \caption{GT, Recon and Heatmap}
    \label{fig:geometry_error}
\end{figure}

\begin{table}[h]
\centering
\caption{Placeholder: Qualitative Comparison with SoTA on the PeopleSnapshot [@cite] dataset and iPER dataset for 3-3 subjects. We report PSNR, SSIM, and LPIPS [@cite] between real images and the images generated by InstantAvatar and two SoTA methods and Anim-NeRF [@cite].}
\begin{tabular}{lllllll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Methods}} & \multicolumn{3}{l}{male-3} & \multicolumn{3}{l}{female-3} \\
\multicolumn{1}{c}{}                         & chamfer    & p2s (gt2pred)   & p2s(pred2gt)   & chamfer    & p2s (gt2pred)   & p2s(pred2gt)     \\
\hline
SelfRecon(2 hour)                   &         &        &         &         &         &          \\
Video Avatars/Octopus(2 hour)                   &         &        &         &         &         &          \\
Vid2Avatar(2 hour)                    &         &        &         &         &         &          \\
Ours(1min)                                        &         &        &         &         &         &          \\
\hline
SelfRecon(10 mins)                   &         &        &         &         &         &          \\
Video Avatars/Octopus(10 mins)                   &         &        &         &         &         &          \\
Vid2Avatar(10 mins)                    &         &        &         &         &         &          \\
Ours(80s)                                        &         &        &         &         &         &          \\
\hline
\end{tabular}
\end{table}

% \subsubsection{Speed} \\

% a. Similar to \ref{fig:speed_comparison} comparing with Anim-Nerf, Instant Avatar and our method.

% b. Create table similar to \ref{tab:speed_comparison}

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/speed_placeholder.png}
%     \caption{Image Quality at different iterations}
%     \label{fig:speed_comparison}
% \end{figure}

% \begin{table}[h]
% \label{tab:speed_comparison}
% \centering
% \begin{tabular}{lcc}
% \toprule
%  & Training & Rendering \\
% \midrule
% Anim-Nerf & 3m 10s & $\sim$ 1 FPS \\
% Instant-Avatar & 1m 47s & $\sim$ 15 FPS \\
% Our & 10s & $\sim$ 300 FPS \\
% \bottomrule
% \end{tabular}
% \end{table}


\subsubsection{Novel Pose Synthesis Quality}\\
a. Qualitative visualization of novel pose \ref{fig:novel_pose}\\
b. Comparison figure with other methods \ref{fig:novel_pose_comparison} \\
c. Create table similar to \ref{tab:novel_pose_comparison}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/novel_pose_placeholder.png}
    \caption{Novel pose synthesis on iPER, People Snapshot and Neuman dataset}
    \label{fig:novel_pose}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/novel_pose_comparison_placeholder.png}
    \caption{Novel pose comparison with Anim-Nerf, Instant Avatar, Video based 3d people}
    \label{fig:novel_pose_comparison}
\end{figure}

\begin{table}[ht]
\centering
\caption{QUANTITATIVE COMPARISON ABOUT NOVEL POSE SYNTHESIS WITH Anim-NeRF, Instant Avatar on iPER and Neuman.}
\label{tab:novel_pose_comparison}
\begin{tabular}{lcccccc}
\toprule
Subject ID & \multicolumn{2}{c}{PSNR$\uparrow$} & \multicolumn{2}{c}{SSIM$\uparrow$} & \multicolumn{2}{c}{LPIPS$\downarrow$} \\
 & NB & OURS & NB & OURS & NB & OURS \\
\midrule
iper-009-4-2 & 20.95 & 24.11 & .9035 & .8927 & .0980 & .0782 \\
iper-023-1-2 & 20.28 & 21.98 & .9009 & .8940 & .0870 & .0644 \\
iper-026-1-2 & 17.42 & 19.27 & .8795 & .8713 & .1192 & .0990 \\
iper-002-1-2 & 19.07 & 23.47 & .8957 & .9165 & .0749 & .0483 \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Mesh Recovery}
SuGaR comparison

\subsection{Ablation Study}

\textbf{Normal Consistency}\\
a. Measure PSNR, LPIPS \ref{tab:ablation}\\
b. Measure P2S and chamfer loss in table

\textbf{Global Scale} \\
a. Measure PSNR, LPIPS \ref{tab:ablation}\\
b. Show faster convergence on subject different than template with image. Similar to \ref{fig:ablation_global_scale}.
\begin{figure}
    \centering
    \includegraphics[width=0.25\linewidth]{figures/ablation_global_scale_placeholder.png}
    \caption{Difference in convergence with the use of global scale}
    \label{fig:ablation_global_scale}
\end{figure}

\textbf{Hash encoded displacement} \\
a. \ref{tab:ablation} \\

\textbf{w/o J optimization} \\
a.table \ref{tab:ablation} \\

\textbf{w/o Pose Refinement} \\
a. table \ref{tab:ablation} \\
b. create figure similar to \ref{fig:ablation_pose_refinement}\\

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/ablation_pose_refinement_placeholder.png}
    \caption{Qualitative Pose improvement with the use of pose refinement}
    \label{fig:ablation_pose_refinement}
\end{figure}

\textbf{Texture Resolution} \\
a. \ref{tab:ablation} \\
b. Create figure similar to \ref{fig:ablation_texture_res}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/ablation_texture_res_placeholder.png}
    \caption{Comparison of view synthesis at different texture resolution}
    \label{fig:ablation_texture_res}
\end{figure}

\begin{table}[ht]
\centering
\caption{Ablation Study for novel view sysnthesis}
\label{tab:ablation}
\begin{tabular}{lcc}
\toprule
Methods & PSNR & LPIPS \\
\midrule
w/o normal map. & - & - \\
w/o hash displacement encoder.      & - & - \\
w/o UV Mapping. & - & - \\
w/o binding gaussians to faces. & - & - \\
Ours & \textbf{-} & \textbf{-} \\
\bottomrule
\end{tabular}
\end{table}

% all units in mm
% subject: male fat
% full chamfer:  v2v:

\begin{table}[]
    \centering
    \caption{Ablation Study for 3d reconstruction}
    \label{tab:ablation}
    \begin{tabular}{lcc}
    \toprule
    Methods & chamfer & p2s \\
    \midrule
    w/o normal map. & - & - \\
    w/o hash displacement encoder.      & - & - \\
    w/o UV Mapping. & - & - \\
    w/o binding gaussians to faces. & - & - \\
    Ours & \textbf{-} & \textbf{-} \\
    \bottomrule
    \end{tabular}
\end{table}

==> sections/methods_backup.tex <==
\section{Method}
\label{sec:method}
Provided a monocular video sequence with a dynamic human and the body poses, our goal is to generate a personalized colored mesh 3D model of a subject consisting of body shape, hair and clothing geometry, and underlying skeleton. Given an $n$ frame video sequence $(I_t)_{t=1}^n$ of a single subject in front of a fixed camera (camera pose and intrinsics), along with the respective body poses $\{\theta_t\}$ we output a personalized animatable representation of the human subject. The keyword `animatable' implies that we should be able to render the underlying representations in novel body poses $\{\theta_j\}$. Additionally, we want to complete the challenging training process in minutes, in favor of scalability.  %TODO: unique trait in 2-3 sentences
    
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/method_pipeline.png}
    \caption{Our method represents the human body in canonical space with gaussians parameterized by 3D gaussian centers $x_c$, rotations $R_c$, scale $S$, opacity $\alpha_o$, skinning weight $w$, global scale $S_g$ and its associated triangle $i_x$. It takes body pose ($\theta_n$) of $n^{th}$ frame as input and applies forward linear blend skinning to transform $x_c$ and $R_c$ to posed space $x_t$ and $R_t$. The normals obtained from the triangular mesh $M(x_c, i_x)$ are encoded to $SH_{\hat{n}}$ and rasterized to obtained normal map. Then, we apply photometric loss and normal map loss to recover both geometry and texture. The normal map ($N_n$) is obtained from monocular RGB image ($I_n$) using pix2pixHD network.}
    \label{fig:method}
\end{figure}

We achieve our goal of obtaining an animatable 3D human using 3D Gaussian Splatting (3D-GS)~\cite{3dgs,guédon2023sugar}. Below we explain the 3D-GS and its deformations as preliminaries in \S \ref{sec:preliminaries}. We then introduce our iHuman representation and describe the details of our method. iHuman consists of initializing 3D-GS in the canonical SMPL pose, see \S \ref{sec:animatable_3d_gaussian}. We bind each 3D Gaussian to a triangle face as described in \S \ref{sec:binding_gaussians_to_mesh_surface}. We then proceed onto deforming the 3D-GS consistent to the posed space, corresponding to the real image in \S \ref{sec:3d_gaussian_deformation}. Taking advantage of explicit 2D Gaussians embedded in 3D~\cite{guédon2023sugar,meshgaussian}, we encode normal for each Gaussian in \S \ref{sec:normal_map_from_3d_gaussian}.

% We first describe the preliminaries that our method is based on in section \ref{sec:preliminaries} which include 3D-GS, pose-guided deformation for deforming 3D Gaussian. Then we introduce our iHuman representation in section \ref{sec:animatable_3d_gaussian}. We deform the 3D Gaussians from canonical to posed space as described in section \ref{sec:3d_gaussian_deformation}. We bind each 3d Gaussian to triangle faces as described in section \ref{sec:binding_gaussians_to_mesh_surface}. Taking advantage of the explicit representation of 3D Gaussian centers, we encode normal for each Gaussian as explained in \ref{sec:normal_map_from_3d_gaussian}. Then, we perform Gaussian Rasterization to render a RGB image and a normal map for given camera parameters and 3d pose.

\subsection{Preliminaries}
\label{sec:preliminaries}
\textbf{3D Gaussian Splatting.}
3D Gaussian Splatting (3D-GS) has recently become the state-of-the-art tool for novel view synthesis. Important for our application, different from NERF, 3D-GS also uses explicit 3D representation using anisotropic 3D Gaussians.

A 3D Gaussian can be written in terms of its full 3D covariance matrix $\Sigma \in \mathbb{R}^{3\times3}, \Sigma \succeq 0$ and position in space $y \in \mathbb{R}^3$ along with center $\mathsf{x} \in \mathbb{R}^3$.
\begin{equation}
\label{eq:std_gaussian}
G(y) = \exp \left(-\frac{1}{2}(y-x)^\top\Sigma^{-1}(y-x)\right).
\end{equation}

Kerbl et al.,~\cite{DBLP:journals/tog/KerblKLD23} however represents each 3D Gaussian to be splatted by the Gaussian 3D center position $x \in \mathbb{R}^3$, color $c \in \mathbb{R}^3$, opacity $\alpha \in \mathbb{R}$, its orientation parametrized by a 3D rotation written as a quaternion $q \in \mathbb{R}^4$, and anisotropic 3D scaling factor $s \in \mathbb{R}^3$~\cite{DBLP:journals/tog/KerblKLD23}. 
\begin{equation}
\label{eq:original_gaussian_representation}
G_p = \{x, q, S, \alpha_0, SH\}.
\end{equation}

Note that Eq.~\eqref{eq:original_gaussian_representation} uses compact sets by approximating Gaussians with ellipsoids, thus simplifying both rendering and optimization \cite{DBLP:journals/tog/KerblKLD23}.
% 3D Gaussian itself is defined by a full 3D covariance matrix $\Sigma$ and a center point $x$ defined in world space, representing the mean value of the Gaussian:
% \begin{equation}
% G(X) = e^{-\frac{1}{2}X^T\Sigma^{-1}X}
% \end{equation}
Nonetheless, equivalence between the two exists where $\Sigma$ can be written explicitly in terms of the scale $s$ and orientation $R(q)$ as:
\begin{equation}
\Sigma = RS S^\top R^\top.
\end{equation}

To project the 3D Gaussians to 2D for rendering, given a viewing transformation $W$, the covariance matrix $\Sigma'$ in camera coordinates is given as follows:

\begin{equation}
\Sigma' = J W \Sigma W^T J^T,
\end{equation}

where, the Jacobian $J$ of the affine approximation of the projective transformation.

The projected Gaussians are depth sorted and rasterized. During the process of rasterization, each Gaussian contributes to the pixel color through an opacity value $\alpha$ and coefficients $\mathbf{c}$ which encapsulate the color information. The resulting volumetric rendering equation that each Gaussian adds to the pixel is represented as follows:

\begin{equation}
C = \sum_{i \in \mathcal{N}} c_i \alpha_i,
\end{equation}

% \textbf{Forward Skinning}

\subsection{Gaussian Human Template Model}
\label{sec:animatable_3d_gaussian}

The human template model is defined by three components:
\begin{equation}
    (M, B, W)
\end{equation}

M is given by:
\begin{equation}
    \label{eq:mesh_verts_and_faces}
    M=(V_c, F)
\end{equation}

where, $V_c=\{x_0, x_1, ..., x_n\}$ is the $n$ number of vertices in canonical space and $F$ is the triangular faces.

$B$ and $W$ are explained in section \ref{sec:3d_gaussian_deformation}.

Different from original 3D Gaussian representation (eq. \ref{eq:original_gaussian_representation}) which works only for the static scene and can produce only the point cloud, we represent our Gaussian based human template model by extending the 3D Gaussian representation with tight integration to $M$ (eq. \ref{eq:mesh_verts_and_faces}).

Our final equation, an extended equation of eq \ref{eq:original_gaussian_representation}, is:
\begin{equation}
G_{\text{skinned}} = \{c, r, s, \alpha, SH, w, \delta_x, i_x\}
\end{equation}
where $w$ is the skinning weights, $\delta_x$ is the vertex displacement, $i_x \in F$ is the parent triangle of $x$. We bind the 3D Gaussians to the parent triangle $i_x$ by centering the gaussian at the centorid of the $i_x$ at $c$. The rotation $r$ and scale $s$ are 2D rotation and scale as explained in \ref{sec:binding_gaussians_to_mesh_surface}.

$c$ is given by: 
\begin{equation}
\label{eq:gaussian_center_from_verts}
    c=\frac{{i_x[1] + i_x[2] + i_x[3]}}{3}
\end{equation}

The displaced $x$ from its initialized position in canonical space is modeled as:
\begin{equation}
x' = x + \delta_x
\end{equation}

We use skinning weights from a standard parametric body model like SMPL \cite{matthew2015smpl} to set $w$.
\\
\textbf{Hash based Displacement and Spherical Harmonics}
% Taken from Animatable 3D Gaussian

\subsection{Binding Gaussians To Mesh Surface}
\label{sec:binding_gaussians_to_mesh_surface}
Similar to SuGaR \cite{guédon2023sugar}, we bind Gaussians to the mesh triangles and optimize the Gaussians and the mesh jointly using the Gaussian Splatting rasterizer.

We associate a single 3D Gaussians at the centroid to each triangle of the original mesh. The Gaussians have only 2 learnable scaling factors instead
of 3 and only 1 learnable 2D rotation encoded with a complex number rather than a quaternion, to keep the Gaussians flat and aligned with the mesh triangles. 

\subsection{3D Gaussian Deformation}
\label{sec:3d_gaussian_deformation}
Given an input pose parameter $\theta_t$, we deform the 3D Gaussians using forward linear blend skinning (equation ...).

The transformation of each point $x$ is calculated with blend skinning $\omega(\theta)$ and target bone transformation $B(\theta_t) = \{B_1(\theta_t), \ldots, B_n(\theta_t)\}$.

The skinning weight field is defined as:
\begin{equation}
w(x_c) = \{w_1, \ldots, w_n\}
\end{equation}
where $x_c$ is a point in canonical space and $n$ is the number of bones.

We transform a point in canonical space to posed space:
\begin{equation}
x_p = \sum_{i=1}^{n} w_i \cdot B_i^t \cdot x'
\end{equation}
where $x_p$ represents the direct mapping of $x'$ in posed space.

From $x_p$, we calculate the 3D Gaussian center $c$ as given in equation \ref{eq:gaussian_center_from_verts} and 3D rotation $q$ from the 2D rotation as explained in section \ref{sec:binding_gaussians_to_mesh_surface}.


\subsection{Normal Map from 3D Gaussian}
\label{sec:normal_map_from_3d_gaussian}
Optimizing 3D gaussians on RGB photometric loss alone cannot recover the intricate details in human body surfaces like facial attributes, wrinkles and hair [See Sup]. So, we take advantage of two crucial facts: \\

i. We have explicit representation of vertices($x_t$) and faces ($i_x$) information for each gaussian to obtain normal of each gaussian without ambiguity \ref{eq: normal_from_faces}.\\

ii. SOTA methods like ECON[@ref ECON] rely on normal map prediction from RGB to produce SOTA results.  \\

So, we use pix2pixHD network to obtain normal map ($I_n$) of every $n$ frame. 

However, obtaining normals directly from gaussian splatting is non trivial. Because of the ambiguity in the depth, we cannot obtain good quality normal map by $\nabla \text{Depth}$. \\

As, we have the triangle associated with each gaussian, we can directly calculate the normals using \ref{eq: normal_from_faces}.

\begin{equation}
    N = \frac{(x_t[i_x[1]] - x_t[i_x[0]]) \times (x_t[i_x[2]] - x_t[i_x[0]])}{\|(x_t[i_x[1]] - x_t[i_x[0]]) \times (x_t[i_x[2]] - x_t[i_x[0]])\|}
    \label{eq: normal_from_faces}
\end{equation}

\( x_c[i_x[j]] \) refers to the \( j \)-th vertex of the triangle in the face \( i_x \). \\

To get normal map from the normal $N$, we encode N as spherical harmonics $SH_\hat{n}$ of degree $0$ by representing $x$, $y$, $z$ component of the normal as $R$, $G$ and $B$ component and converting to $SH_\hat{n}$.

\begin{equation}
    {SH_\hat{n}} = \frac{1}{\sqrt{4\pi}} \begin{bmatrix} R \\ G \\ B \end{bmatrix}
\end{equation}

We do another pass in gaussian rasterizer to obtain the normal map ($I_{\hat{n}}w$).


% \subsection{Joint Appearance and Pose Optimization}
% Present 3D pose estimation ($\theta$, translation $(t)$) methods like [@cite Vibe, ROMP] cannot provide accurate pose. Using those poses for reposing Gaussian and optimizing doesn’t result in an output that models the body shape accurately.

% The inaccurate pose input impacts the alignment of the rendered model with the image, leading to unsatisfactory rendering outcomes.

% To address this issue, we propose an optimization approach for the pose parameters $\theta_t$. We set the $\theta_t$ as an optimization parameter and initialize it using the initial prediction from the pose regression model.

\subsection{Training Loss}
We use the combination of L1 and D-SSIM term for both photometric loss and normal map loss. 

We also use normal consistency regularizer.
